Robust and Accurate -- Compositional Architectures for Randomized Smoothing

Randomized Smoothing (RS) is considered the state-of-the-art approach to obtain certifiably robust models for challenging tasks. However, current RS approaches drastically decrease standard accuracy on unperturbed data, severely limiting their real-world utility. To address this limitation, we propose a compositional architecture, ACES, which certifiably decides on a per-sample basis whether to use a smoothed model yielding predictions with guarantees or a more accurate standard model without guarantees. This, in contrast to prior approaches, enables both high standard accuracies and significant provable robustness. On challenging tasks such as ImageNet, we obtain, e.g., $80.0\%$ natural accuracy and $28.2\%$ certifiable accuracy against $\ell_2$ perturbations with $r=1.0$. We release our code and models at https://github.com/eth-sri/aces.

==> related_work.tex <==
\section{Related Work}

In this section we briefly review related approaches.

\paragraph{Adversarial Robustness}
We distinguish between probabilistic and deterministic approaches to certified robustness to adversarial examples.
Deterministic certification methods compute the reachable set for given input specifications using convex relaxations \citep{GehrMDTCV18, ZhangWCHD18, WangPWYJ18, WengZCSHDBD18, WongK18, singh2018fast,singh2019abstract,xu2020automatic,muller2021prima},
mixed integer linear programming \citep{tjeng2017evaluating}, semidefinite programming \citep{RaghunathanSL18a, dathathri2020enabling}, or satisfiability modulo theories \citep{katz2017reluplex, Ehlers17}, to then reason about properties of the output.
To obtain networks amenable to such approaches, specialized training methods have been proposed
\citep{RaghunathanSL18b, MirmanGV18, GowalDSBQUAMK18, BalunovicV20,xu2020automatic}.
However, while these methods can provide state-of-the-art guarantees for $\ell_{\infty}$ robustness specifications, they are computationally expensive, limited to networks of small sizes and tend to perform poorly on $\ell_1$ and $\ell_{2}$ specifications.

Probabilistic certification construct a robustified classifier by \citep{LiCWC19, LecuyerAG0J19, CohenRK19} introducing noise to the classification process to obtain probabilistic robustness guarantees, allowing the certification of larger models than deterministic methods.
We review \citet{CohenRK19}
in \cref{sec:randomized-smoothing}.%

\paragraph{Robustness-Accuracy Trade-Off}
Most provable and heuristic defenses focus on maximizing the provable or empirically robust accuracy, leading to a significant drop in performance on unperturbed samples, which has limited their real world impact and sparked an analysis of the fundamental trade-off between robustness and accuracy \citep{zhang2019theoretically,XieTGWYL20,Raghunathan19AdvCanHurt}. 
Some heuristic defenses such as \trades \cite{zhang2019theoretically} have introduced a principled way to control this trade-off, by modifying the composition of the loss function during training. However these approaches require retraining the whole network to obtain a different trade-off, making the exploration of the pareto curve expensive and adaptively changing the focus between robustness and accuracy during the deployment of a model impractical.
\todo{smoothing papers in this realm}


More recently \citet{mueller2021certify} introduced a compositional architectures for certification (ACE) which leverages two independent models, one robust and one highly accurate by combining them with a certifiable, parametrized selection mechanism to decide at inference time which of the two to use. This not only allows exploring the full pareto-cure without any retraining but also for the first time yields models with very high natural accuracy and a reasonable amount of certifiable robustness.


==> test-section.tex <==
\section{Test Section} \label{sec:test}

Interesting stuff:

\begin{itemize}
	\item Citations are set up already: Turing~\cite{turing1937computable}
	\item You may use UTF-8 characters: ä
	\item Use cref for references: \cref{sec:test}
	\item Reference the appendix by a custom command: \App{app:xyz} and \app{app:xyz}.
	\item Use the \texttt{acro} package for acronyms: First usage: \ac{cli}, subsequent usages: \ac{cli}
\end{itemize}

\begin{figure}
	\centering
	An example figure content.
	\caption{An example figure caption.}
	\label{fig:example}
\end{figure}

\paragraph{Figures}
See \cref{fig:example} for an example figure.

\lstinputlisting[caption={Example code.},label=lst:code]{code/example-code.psi}

\paragraph{Listings}
See \cref{lst:code} for an example Listing.




